SILENT: A New Lens on Statistics in Software Timing Side Channels

Cryptographic research takes software timing side channels seriously. Approaches to mitigate them include constant-time coding and techniques to enforce such practices. However, recent attacks like Meltdown [42], Spectre [37], and Hertzbleed [70] have challenged our understanding of what it means for code to execute in constant time on modern CPUs. To ensure that assumptions on the underlying hardware are correct and to create a complete feedback loop, developers should also perform \emph{timing measurements} as a final validation step to ensure the absence of exploitable side channels. Unfortunately, as highlighted by a recent study by Jancar et al. [30], developers often avoid measurements due to the perceived unreliability of the statistical analysis and its guarantees. In this work, we combat the view that statistical techniques only provide weak guarantees by introducing a new algorithm for the analysis of timing measurements with strong, formal statistical guarantees, giving developers a reliable analysis tool. Specifically, our algorithm (1) is non-parametric, making minimal assumptions about the underlying distribution and thus overcoming limitations of classical tests like the t-test, (2) handles unknown data dependencies in measurements, (3) can estimate in advance how many samples are needed to detect a leak of a given size, and (4) allows the definition of a negligible leak threshold $\Delta$, ensuring that acceptable non-exploitable leaks do not trigger false positives, without compromising statistical soundness. We demonstrate the necessity, effectiveness, and benefits of our approach on both synthetic benchmarks and real-world applications.

==> sections/06b-old-real-world.tex <==

To demonstrate the effectiveness of our approach, we illustrate how the algorithm would perform in different security fields in which software timing side channels pose a potential threat. At the same time, we expect that the example use cases we consider should come with varying degrees of variance and both significant and minor side channels.
\subsection{Considered Security Fields}

\paragraph{Symmetric Cryptography: AES}
To evaluate how our algorithm would perform in the analysis of symmetric primitives, for which we considered the examples that are provided by dudect\cite{dudect16}. Dudect provides a 32-bit AES software implementation using T-tables, as well as an AES implementation by Emilia Käsper and Peter Schwabe\cite{CHES:KasSch09}, which uses a bit-slicing approach\cite{bitsliceaes}. The 32-bit T-table implementation is known to be vulnerable\cite{Bernstein2005CachetimingAO}, while the bit-slicing implementation has no known weaknesses. 
%We measured both implementations in a low variance environment with CPU isolation enabled, resulting in relatively clean, discrete measurements.

\paragraph{Asymmetric Cryptography: X25519}
To evaluate our approach against classic asymmetric algorithms, we similarly tested our algorithms against the X25519 implementation 'donna' from Adam Langley\footnote{\url{https://github.com/agl/curve25519-donna}}, which is included in the dudect examples.
Additionally, we consider the purposefully vulnerable variant 'donna-bad', which is also part of the dudect examples and contains an obvious side-channel. The implementation from Adam Langley has no known vulnerabilities.


\paragraph{Post Quantum Cryptography: Kyber}
To evaluate our approach on post-quantum primitives, we tested the reference implementation of Kyber, a post-quantum key encapsulation mechanism, for the Kyberslash 1 vulnerability~\cite{bernstein2025kyberslash}. Kyberslash 1 exploits runtime differences of secret-dependent division operations included when compiling the reference code for smallest code size on certain platforms. 

\paragraph{Cryptopgraphic Protocols: TLS}
In order to test our approach against a more practical remote scenario, we evaluated our approach against TLS libraries regarding the Lucky13 attack, Bleichenbachers attack and the CBC Padding Oracle attack. For this purpose, we reused the public data set of Dunsche et al.\cite{rtlf}, which gathered the data in a semi-remote scenario. Here, we focus on the data set collected for the \textit{mbedTLS} library as it highlights an issue of real-world measurements: dependence between measurements.
\todo{NE: Alle 3 Angriffe? In der Tabelle haben wir bisher nur einen betrachtet.}

\paragraph{Security: Web Application}
To demonstrate the potential of our tool in the context of web application penetration tests, we developed and evaluated a small Flask application written in Python.
The application simulates a simple user authentication check. When run for the first time, it creates a SQLite database containing 1000 pre-registered users. It then exposes a single endpoint that evaluates the \texttt{Authorization} header\footnote{The \texttt{Authorization} header can be used to provide credentials that authenticate a user with a server, allowing access to protected resources.}. If a username is provided, the application queries the database to determine whether the user exists. Regardless of the query result, the response is always identical, which hides internal processing.
Our server is inspired by the work\footnote{\url{https://portswigger.net/research/listen-to-the-whispers-web-timing-attacks-that-actually-work}} of James Kettle. He showed that when specific headers are set in a request, some servers take longer to respond.
For this security field we consider different measurement scenarios. First, we perform local measurements on the same system where the server runs. Next, we conduct LAN measurements from a system connected by cable to the server. Finally, we conduct Internet measurements, we measure from within the same country and from a more distant different country.
\todo{NE: Rewriten wenn Server final ist...}

% \begin{lstlisting}[caption={Relevant code part illustrating the webserver's simple authentication check.}, label={lst:webserver-auth}, frame=tb, numbers=left, breaklines=true, basicstyle=\scriptsize\ttfamily]
% def check_user(username):
%     with sqlite3.connect(DATABASE) as conn:
%         row = conn.execute("SELECT id FROM users WHERE username = ?", (username,)).fetchone()

% @app.route("/")
% def index():
%     username = request.headers.get("Authorization")
%     if username:
%         check_user(username)
%     return "Welcome to our service!"
% \end{lstlisting}

% \begin{lstlisting}[caption={Relevant code part illustrating the webserver's basic logging process.}, label={lst:webserver-logging}, frame=tb, numbers=left, breaklines=true, basicstyle=\scriptsize\ttfamily]
% def log_user(username):
%     with open(LOGFILE, "a") as f:
%         f.write(f"{datetime.now()} - Authorization={username}\n")

% @app.route("/")
% def index():
%     username = request.headers.get("Authorization")
%     if username:
%         log_user(username)
%     return "Welcome to our service!"
% \end{lstlisting}


\subsection{Collecting Measurements and Choosing the Sample Size}
For AES, X25519, and Kyber, we collect measurements using existing implementations and tools from related work to achieve comparable results. For mbedTLS, we directly use the data set from \cite{rtlf}. Finally, for our web applications use case, we built a demo application with a controlled time leak through database accesses. We provide more details on how we collected measurements in \todo{cite appendix}.
To determine a suitable sample size, we use our methodology from \todo{Ref}. To obtain a first assessment, we applied our estimation based on an initial sample size of 100 measurements for all examples. We set our parameters to achieve a detection rate of 90\% and to allow a false positive rate of 1\%. We further set an estimate for the expected size of the timing leak guided by previous studies on the considered implementations~\cite{dudect16, bernstein2025kyberslash, bernstein2005cache}. Specifically, for the AES example, we set the expected timing difference to be 0.2 cycles as the leak depends on the cache and hence does not affect all measurements. For the modified x25519 implementation, we set an expected difference of 5 cycles. For Kyber, we set an expected difference of 20 cycles based on the results of the Kyberslash paper. \todo{add mbedtls} Finally, for the web application, we assumed a large leak of 340,000 cycles based on the access time of the utilized database. We further set $\Delta$ in relation to the size of the respective side channel. For example, we set $\Delta$ to be 0.1 for AES and 10,000 for the web application case. Note that due to the varying distribution of the measurements and expected side channel sizes, this results in distinct sample size shown in \autoref{tab:realWorldEval-results}: for example, for Kyberslash, we estimate a required sample size of 1368, while for the web application exmaple, we only require 127 in a LAN environment. Based on these prescribed sample sizes, we then collected measurements and tested if we are able to detect the timing difference. Additionally, we compared the measurements of one distribution to test for false positives. Since Kyberslash provides a comparatively small but consistent side channel, we additionally conducted 1,000 repetitions of our measurements to study if our estimation of the sample size actually leads to a detection rate close to the sought rate of 90\%.

\subsection{Results}
As shown in \autoref{tab:realWorldEval-results}, we were able to detect the expected leaks for all use cases using the estimated sample size. For the initial 100 samples, in contrast, we have not been able to detect any leaks yet, except for the modified x25519 example. Based on the particularly distinct timing difference we measured, we assume our initial estimation of the size of leak to be too conservative. We further found that the measurements of x25519 and AES with bit slicing exhibit a distinct level of dependence between the obtained measurements. This could both be attributed to the code or the measurement setup of the two examples. As described before, the mbedTLS data set also shows a high level of dependence. In contrast to the test performed by Dunsche et al.~\cite{rtlf}, our test did not indicate a timing leak for the initial or estimated sample size. Since their work could not find evidence for a timing leak in the source code and thus already assumed their result to be false positive, we believe that this was likely due to the strong dependence of the data which is not considered by their RTLF.

\paragraph{Sample Size Estimation and $\Delta$} Our 1,000 repetitions of the Kyberslash measurements with a sample size of 1368 had an overall detection rate of 80.2\%. While we were aiming for a detection rate of did 90\%, we still consider this to be a good result given that our power analysis only yields a rough estimate for the required sample size. We further analyzed the 1,000 measurements using $\Delta = 20$ to evaluate the effect of our threshold on real-world measurements. We noticed that around \todo{10\%} of the measurements indicated a notably higher difference than expected. We attribute these prolonged leaks to side effects of the system caused by background processes and their interaction with the scheduler, RAM, and CPU cache. Effectively, our $\Delta$ threshold was hence not always sufficient. In total, we detected a leak exceeding $\Delta$ \todo{\$howOften} times.

==> tables/artificialScenarios-rejectionRates.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c | ccccc}
        \textbf{Scenario} & \textbf{\gls{normal}} & \textbf{\gls{indAR-}} & \textbf{\gls{indAR+}} & \textbf{\gls{dep-}} & \textbf{\gls{dep+}}\\\hline
          & \multicolumn{5}{c}{\textbf{$\mu=0$}}\\\hline
        \textit{\gls{irtlf}} $\alpha$ &0.0019& 0  &0&0&0\\
        \textit{\gls{rtlf}} $\alpha$&0.0458&0.0184&0.2373&0.018&0.2128\\
        \textit{t-test} $\alpha$&  0.101& 0.0044 &0.3428& 0.0028&0.316\\
        \textit{paired t-test}  $\alpha$& 0.1014 & 0.0043 & 0.3446& 0.0051&0.3372\\
        \hline
          & \multicolumn{5}{c}{\textbf{$\mu=\Delta/2$}}  \\\hline
          \textit{\gls{irtlf}}& 0.01& 0.0006&0.0018&0.0004&0.0023\\
        \textit{\gls{rtlf}} & 0.1564 & 0.8361&0.6842&0.8432&0.6768\\
        \textit{t-test} & 0.3055 & 0.9931 &0.7933&0.9952&0.8021\\
        \textit{paired t-test}  &0.3059 & 0.9932 &0.793&0.9968&0.8135\\
          \hline
                 & \multicolumn{5}{c}{\textbf{$\mu=0.95\Delta$}}\\\hline
        \textit{\gls{irtlf}} &0.0584& 0.0634  &0.0729&0.0666&0.0701\\
        \textit{\gls{rtlf}} & 0.4309 & 1 &0.9727&1&0.9787\\
        \textit{t-test} & 0.6811 & 1 &0.9918&1&0.9943\\
        \textit{paired t-test}  & 0.6817  & 1  &0.9917& 1&0.9949 \\
        \hline
          & \multicolumn{5}{c}{\textbf{$\mu=\Delta$}}  \\\hline
        \textit{\gls{irtlf}}& 0.0706 &0.1094&0.0943&0.1124&0.095\\
        \textit{\gls{rtlf}} & 0.4615  & 1&0.9816&1&0.9855\\
        \textit{t-test} & 0.7211  & 1&0.9954&1&0.9963\\
        \textit{paired t-test}  & 0.7217 & 1 &0.9952&1&0.9968\\
          \hline
          & \multicolumn{5}{c}{\textbf{$\mu=2\Delta$} } \\\hline
        \textit{\gls{irtlf}} &0.6697 &1&0.9754&1&0.9824\\
        \textit{\gls{rtlf}} & 0.9706 & 1&0.9997&1&1\\
        \textit{t-test} & 0.9967 & 1&0.9998&1&1\\
        \textit{paired t-test}  & 0.9967 & 1 &0.9998&1&1\\
    \end{tabular}
    \caption{Table with rejection rates $\hat\alpha$ for $\alpha=0.1$.}
    \label{tab:artificial_example}
\end{table}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{lcccc}
%         \toprule
%          \textbf{Tools} & \textbf{\gls{ind}} & \textbf{\gls{bias}} & \textbf{\gls{dep+}} & \textbf{\gls{dep-}}\\
%         \midrule
%         \gls{irtlf}       & 0.094 & 0.076 & 0 & 0.001\\
%         \gls{rtlf}     & 0.223 & 0.209 & 0 & 0.188 \\
%         t-test       & 0.656 & 0.693 & 0.822 & 0.846\\
%         paired t-test    & 0.654& 0.693 & 1 & 0.737 \\
%         \gls{rtlf} modified     & - & 0.209 & - & -\\
%         \bottomrule
%     \end{tabular}
%     \caption{Table with rejection rates for $\alpha=0.1$. \gls{rtlf} mod corresponds to \gls{rtlf} and only rejecting whenever the signal is greater than $\frac{1}{n^{1/4}}$}
%     \label{tab:artificial_example}
% \end{table}

==> tables/artificialScenarios.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{ll}
        \toprule
        \textbf{Scenario} & \textbf{Description}\\
        \midrule
        \textbf{\gls{normal}} & $X_n$, $Y_n$ independent standard normal \\
        \textbf{\gls{indAR+}} & $X_n,Y_n$ independent AR(1) with $\phi=0.5$\\
        \textbf{\gls{indAR-}} & $X_n,Y_n$ independent AR(1) with $\phi=-0.5$\\
        \textbf{\gls{dep-}} & $X_n,Y_n$ positive correlated AR(1) with $\phi=-0.5$ \\
        \textbf{\gls{dep+}} & $X_n,Y_n$ positive correlated AR(1) with $\phi=0.5$\\
        \bottomrule
    \end{tabular}
    \caption{TODO}
    \label{tab:scenarios}
\end{table}

==> tables/realWorlEval-results.tex <==
\begin{table*}[t]
    \centering
    \small
    \caption{$\alpha=0.1$ \todo{$0.01$} \todo{Diese Tabelle fliegt raus, da Tabelle 2 und 3 vorhanden.}}
    \begin{tabular}{llcccccc}
        \toprule
        \textbf{Security Field} & \textbf{Algorithm} 
        & \makecell[c]{\textbf{Dependence}\\ \textbf{$m$}}
        & \makecell[c]{\textbf{Samples}\\ \textbf{$n$}}  
        & \makecell[c]{\textbf{Threshold}\\ \textbf{$\Delta$}}
        & \makecell[c]{\textbf{Expected}\\ \textbf{Difference}}
        & \makecell[c]{\textbf{Expected}\\ \textbf{Result}} 
        & \makecell[c]{\textbf{Evaluated}\\ \textbf{Result}} \\
        \midrule
        Symmetric Cryptography & AES with Bit Slicing & 5 & 100 & 0.1 & - & \faSlash & - \\
                               & AES with Bit Slicing & 846 & 79381 & 0.1 & 0.2 & \faSlash & 2.1 \todo{issue} \\
                               & AES with T-Table & 2 & 100 & 0.1 & 0.2 & \faStopwatch & - \\
                               & AES with T-Table & 1 & 89906 & 0.1 & 0.2 & \faStopwatch & 0.198 \\
        \midrule
        Asymmetric Cryptography & x25519-donna & 2 & 100 & 0.1 & 5 & \faSlash & - \\
                                & x25519-donna & 345  & 83740 & 0.1 & 5 & \faSlash & - \\
                                & x25519-donna bad & 11 & 100 & 0.1 & 5 & \faStopwatch & 7600.9 \\
                                & x25519-donna bad & 964 & 371843 \todo{maybe cut}& 0.1 & 5  & \faStopwatch & 6636 \\
        \midrule
        Post Quantum Cryptography & Kyber (speed optimized) & 1 & 100 & 5 & - & \faSlash & - \faSlash \\
                                  & Kyber (speed optimized) & 6 & 1368 & 5 & - & \faSlash & - \faSlash \\
                                  & Kyber (size optimized) & 2 & 100 & 5 & 20 & \faStopwatch & - \textcolor{red}{\faSlash} \\
                                  & Kyber (size optimized) & 10 & 1368 & 5 & 20 & \faStopwatch & 32 \faStopwatch \\
        \midrule
        Cryptopgraphic Protocols & \gls{mbedtls} with TLS & 9 & 100 & 50 & 100 & \faSlash & - \\
                                 & \gls{mbedtls} with TLS & 2122 & 107431941 & 50 & 100 & \faSlash & -
                                 \\
        \midrule
        Web Application & Local & 2 & 100 & 5 & 41700 & \faStopwatch & - \\
                 & Local & 2 & 505 (1000) & 5 & 41700 &  \faStopwatch & 92140 \\
                 & LAN & 1 & 100 & 5 & 41700 & \faStopwatch & - \\
                 & LAN & 3 & 698 (1000) & 5 & 41700 &  \faStopwatch & 85108 \\
                 & Internet (same country)  & 2 & 100 & 5 & 24300 & \faStopwatch & - \\
                 & Internet (same country) & 37 & 7941 (5000) & 5 & 24300 &  \faStopwatch & 74722  \\
                 & Internet (different country) & 2 & 100 & 5 & 67680 & \faStopwatch & - \\
                 & Internet (different country) & ? & 112411 (250000) & 5 & 67680 &  \faStopwatch & ? \\
        \midrule
        \multicolumn{8}{c}{\faStopwatch~Difference \hspace{5mm} \faSlash~No Difference}\\
        \bottomrule
    \end{tabular}
    \label{tab:realWorldEval-results}
\end{table*}

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{llcccccc}
%         \toprule
%         \textbf{Scenario} & \textbf{Algorithm} & \makecell[c]{\textbf{Dependence}\\ \textbf{$m$}}& \textbf{$n$} & \textbf{$\Delta$}&  \makecell[c]{\textbf{Expected}\\ \textbf{Result}} & \makecell[c]{\textbf{Evaluated}\\ \textbf{Result}} \\
%         \midrule
%         Symmetric Cryptography & AES T-Table & & & & \\
%                                & AES Bit Slicing & & & & \\
%         \midrule
%         Asymmetric Cryptography & x25519-donna & 851 & 849643 & 100 & & \textcolor{green}{\scalebox{1.5}{\ding{51}}} \\
%                                 & x25519-donna bad & 2131 & 504307 & 100 & Difference & \textcolor{green}{\scalebox{1.5}{\ding{51}}} \\
%         \midrule
%         Post Quantum Cryptography & Kyberslashdiff & 2 & 100 & 5 & Difference & \textcolor{red}{\scalebox{1.5}{\ding{55}}} \\
%          & Kyberslashnodiff & 1 & 100  & 5 & No Difference & \textcolor{green}{\scalebox{1.5}{\ding{51}}} \\    
%         & Kyberslashdiff & 5 & 1000 & 5 & Difference & \textcolor{green}{\scalebox{1.5}{\ding{51}}}\\
%          & Kyberslashnodiff & 15 & 1000  & 5 & No Difference & \textcolor{green}{\scalebox{1.5}{\ding{51}}} \\
%         \midrule
%         Web Applications & Webserverxx & 3 & 100 & 100 & No Difference & \textcolor{green}{\scalebox{1.5}{\ding{51}}} \\
%          & Webserveryy & 3 & 100 & 100 & No Difference & \textcolor{green}{\scalebox{1.5}{\ding{51}}}\\
%          & Webserverxy & 2 & 100 & 100 & Difference & \textcolor{green}{\scalebox{1.5}{\ding{51}}}\\
%          & Webserverxx & 21 & 1000 & 100 & No Difference & \textcolor{green}{\scalebox{1.5}{\ding{51}}} \\
%         & Webserveryy & 21 & 1000 & 100 & No Difference & \textcolor{green}{\scalebox{1.5}{\ding{51}}} \\
%          & Webserverxy & 7 & 1000 & 100 & Difference & \textcolor{green}{\scalebox{1.5}{\ding{51}}}\\
%         \bottomrule
%     \end{tabular}
%     \caption{$\alpha=0.1$}
%     \label{tab:realWorldEval-results}
% \end{table*}
